Characterizing Rothe Diagrams

Rothe diagrams are diagrams which track inversions of a permutation. We define six main properties that Rothe diagrams fulfill: the southwest, dot, popping, numbering, step-out avoiding, and empty cell gap rules. We prove that -- given an arbitrary bubble diagram -- four different subsets of these properties provide sufficient criteria for the diagram to be a Rothe diagram. We also prove that when a set of ordered, freely floating, non-empty columns satisfy the numbering and step-out avoiding rules, then they can be arranged into a Rothe diagram.

==> Archive/sami.tex <==

%%%%%%%%%%%%%%%%%%%%%%
% macreau for tableaux
%%%%%%%%%%%%%%%%%%%%%%
\newlength\cellsize \setlength\cellsize{8\unitlength}

\savebox2{% BOX
\begin{picture}(8,8)
\put(0,0){\line(1,0){8}}
\put(0,0){\line(0,1){8}}
\put(8,0){\line(0,1){8}}
\put(0,8){\line(1,0){8}}
\end{picture}}

\newcommand\boxify[1]{\def\thearg{#1}\def\nothing{}%
\ifx\thearg\nothing\vrule width0pt height\cellsize depth0pt%
  \else\hbox to 0pt{\usebox2\hss}\fi%
  \vbox to \cellsize{\vss\hbox to \cellsize{\hss$_{#1}$\hss}\vss}}

\savebox3{% CIRCLE
\begin{picture}(8,8)
\put(4,4){\circle{8}}
\end{picture}}

\newcommand{\circify}[1]{\def\thearg{#1}\def\nothing{}%
\ifx\thearg\nothing\vrule width0pt height\cellsize depth0pt%
  \else\hbox to 0pt{\usebox3\hss}\fi%
  \vbox to \cellsize{\vss\hbox to \cellsize{\hss$_{#1}$\hss}\vss}}

\newcommand\nullify[1]{\def\thearg{#1}\def\nothing{}%
\ifx\thearg\nothing\vrule width0pt height\cellsize depth0pt%
  \else\hbox to 0pt{\hss}\fi%
  \vbox to \cellsize{\vss\hbox to \cellsize{\hss$_{#1}$\hss}\vss}}


\newcommand\tableau[1]{\vtop{\let\\=\cr
\setlength\baselineskip{-8000pt}
\setlength\lineskiplimit{8000pt}
\setlength\lineskip{0pt}
\halign{&\boxify{##}\cr#1\crcr}}}

\newcommand\cirtab[1]{\vline\vtop{\let\\=\cr
\setlength\baselineskip{-8000pt}
\setlength\lineskiplimit{8000pt}
\setlength\lineskip{0pt}
\halign{&\circify{##}\cr#1\crcr}}}

\newcommand\nulltab[1]{\vtop{\let\\=\cr
\setlength\baselineskip{-8000pt}
\setlength\lineskiplimit{8000pt}
\setlength\lineskip{0pt}
\halign{&\nullify{##}\cr#1\crcr}}}

\savebox2{% BOX
\begin{picture}(8,8)
\put(0,0){\line(1,0){8}}
\put(0,0){\line(0,1){8}}
\put(8,0){\line(0,1){8}}
\put(0,8){\line(1,0){8}}
\end{picture}}

\newcommand{\csix}{red}
\newcommand{\cfiv}{orange}
\newcommand{\cfou}{yellow}
\newcommand{\cthr}{green}
\newcommand{\ctwo}{blue}
\newcommand{\cone}{violet}


\newcommand{\cball}[2]{%
  \begin{tikzpicture}
    \filldraw[fill=#1!35,draw=black] (0,0) circle (4pt) node {$\scriptstyle #2$};
  \end{tikzpicture}
}

\newcommand{\cbox}[2]{%
  \begin{tikzpicture}
    \draw +(-4pt,-4pt) rectangle +(4pt,4pt);
    \node (0,0) {$\scriptstyle \mathbf{#2}$};
  \end{tikzpicture}
}

\newcommand{\leftball}[2]{\makebox[0pt]{\raisebox{1.5pt}{$\leftarrow$}}\cball{#1}{#2}}

\begin{document}

\begin{figure}[ht]
  \begin{center}
    \begin{tikzpicture}[xscale=1.2,yscale=0.8]
      \node at (0,5) (A) {$\cirtab{ ~ \\ ~ & ~ \\ \\\hline}$};
      \node at (1,4) (B) {$\cirtab{ ~ \\ ~ \\ & ~ \\\hline}$};
      \node at (2,3) (C) {$\cirtab{ ~ \\ \\ ~ & ~ \\\hline}$};
      \node at (1,2) (E) {$\cirtab{ \\ ~ \\ ~ & ~ \\\hline}$};
      \node at (0,3) (H) {$\cirtab{ \\ ~ & ~ \\ ~ \\\hline}$};
      \draw[thin] (A) -- (H) ;
      \draw[thin] (A) -- (B) ;
      \draw[thin] (H) -- (E) ;
      \draw[thin] (B) -- (E) ;
      \draw[thin] (B) -- (C) ;
      \draw[thin] (C) -- (E) ;
      \node at (4,5) (A2) {$\vline\tableau{3 & 2 \\ 2 \\ & \\\hline}$};
      \node at (5,4) (B2) {$\vline\tableau{3 & 1 \\ 2 \\ & \\\hline}$};
      \node at (6,3) (C2) {$\vline\tableau{3 & 1 \\ 1 \\ & \\\hline}$};
      \node at (5,2) (E2) {$\vline\tableau{2 & 1 \\ 1 \\ & \\\hline}$};
      \node at (4,3) (H2) {$\vline\tableau{2 & 2 \\ 1 \\ & \\\hline}$};
      \draw[thin] (A2) -- (H2) ;
      \draw[thin] (A2) -- (B2) ;
      \draw[thin] (H2) -- (E2) ;
      \draw[thin] (B2) -- (E2) ;
      \draw[thin] (B2) -- (C2) ;
      \draw[thin] (C2) -- (E2) ;
    \end{tikzpicture}
    \caption{\label{fig:kohnert}The set $\KD(0,2,1)$ of Kohnert diagrams for $(0,2,1)$ and their images under the injection with reverse tableaux.}
  \end{center}
\end{figure}

\end{document}

==> Archive/unuseddigrams.tex <==
\begin{figure}[ht]
  \begin{displaymath}
    \arraycolsep=0.9\cellsize
    \begin{array}{ccc}
      \nulltab{
        \\
        \put(4,0){\line(0,1){8}} \\
        \put(4,0){\line(0,1){8}} \\
        \put(4,0){\line(0,1){8}} \\
        \put(4,0){\line(0,1){8}} \\
        \put(4,0){\line(0,1){8}} \\
      }
      \nulltab{
        \usebox3 \put(-8,0){\line(1,0){8}} \\
        \usebox3 \put(-8,0){\line(1,0){8}} \\
        \usebox3 \put(-8,0){\line(1,0){8}} \\
        \cball \\
        \usebox3 \put(-8,0){\line(1,0){8}} \\
        \cball \put(-8,0){\line(1,0){8}} \\
      }
      \boxtab{ 
        
        \put(-4,-6.5){\line(1,0){8}} & \put(-4,-6.5){\line(1,0){8}} & \usebox3 & \usebox3 & & & \cball & & \\
        \put(-4,-6.5){\line(1,0){8}} & \put(-4,-6.5){\line(1,0){8}} & \put(0,0){\line(0,1){8}} \usebox3 & \cball & & & & \\
        \put(-4,-6.5){\line(1,0){8}} & \put(-4,-6.5){\line(1,0){8}} & \put(0,0){\line(0,1){8}} \usebox3 & \usebox3 & & \usebox3 & \cball & \\
        & b & \put(-4,0){\line(0,1){8}} & & \\
        \put(-4,-6.5){\line(1,0){8}} & \usebox3 & \put(0,0){\line(0,1){8}} \usebox3 & \cball & \\ 
        a & \put(-4,0){\line(0,1){8}} & \put(-4,0){\line(0,1){8}} \\\hline }
      
    \end{array}
  \end{displaymath}
  \caption{\label{fig:ecg_main}The main diagram showing the empty cell gap rule is satisfied.}
\end{figure}

\begin{figure}[ht]
\begin{center}
\begin{tikzpicture}[scale=0.3]
\def\rows{6} %number of rows
\def\cols{6} %number of columns
  \draw[-](0,0) -- (\rows,0); %axes
  \draw[-](0,0) -- (0,\cols); 
  \foreach \x/\y in {1/3,2/2,3/1,6/5} { %dot positions
    \draw[fill=black] (\x-0.5,\y-0.5) circle(0.2);
  %line positions
    \draw[-latex](\x-0.5,\y-0.5) -- (\x-0.5,6.7); }
  \foreach \x/\y in {1/1,1/2,2/1,5/5} %circle positions
    \draw (\x-0.5,\y-0.5) circle(0.5);
\end{tikzpicture}
  \caption{\label{fig:bad_va}A bubble diagram which satisfies the bubble popping rule, but is not a permutation diagram.}
\end{center}
\end{figure}

\begin{figure}[ht]
  \begin{displaymath}
    \arraycolsep=0.9\cellsize
    \begin{array}{cc}
      \boxtab{ 
        & & \usebox7 \\
        & \usebox7 & \\
        \usebox7 & & \\
        \usebox3 & \usebox3 & \usebox3 & \usebox7 & \\
        & & & \usebox3 & \usebox7 \\\hline } &
      
    \end{array}
  \end{displaymath}
  \caption{\label{fig:bad_dot}A bubble diagram which satisfies the dot condition, but is not a permutation diagram.}
\end{figure}

\begin{figure}[ht]
  \begin{displaymath}
    \arraycolsep=0.9\cellsize
    \begin{array}{c}
      \cirtab{ 
        & & 4 & 5 & \\
        & & 3 \\
        & 2 \\
        & \\\hline}
      
    \end{array}
  \end{displaymath}
    \caption{\label{fig:bad_number}A bubble diagram which satisfies the numbering condition yet is not a permutation diagram.}
\end{figure}

==> temp_notes.tex <==
replace position with cell
make sure that Rothe Diagrams are explained to be the same as permutation/inversion diagrams


Random sorting networks by Angel 06/07 uses permutation matricies (if we have time to add info about it)
